Free probability, path developments and signature kernels as universal scaling limits

Random developments of a path into a matrix Lie group $G_N$ have recently been used to construct signature-based kernels on path space. Two examples include developments into GL$(N;\mathbb{R})$ and $U(N;\mathbb{C})$, the general linear and unitary groups of dimension $N$. For the former, [MLS23] showed that the signature kernel is obtained via a scaling limit of developments with Gaussian vector fields. The second instance was used in [LLN23] to construct a metric between probability measures on path space. We present a unified treatment to obtaining large $N$ limits by leveraging the tools of free probability theory. An important conclusion is that the limiting kernels, while dependent on the choice of Lie group, are nonetheless universal limits with respect to how the development map is randomised. For unitary developments, the limiting kernel is given by the contraction of a signature against the monomials of freely independent semicircular random variables. Using the Schwinger-Dyson equations, we show that this kernel can be obtained by solving a novel quadratic functional equation. We provide a convergent numerical scheme for this equation, together with rates, which does not require computation of signatures themselves.

==> Numerical_Scheme/spare.tex <==

% Throughout this section, we assume that $\gamma:[s,t]\to V$ is a piecewise linear path on some partition $\PP_0 = \{s=t_0\leq t_1\leq \dots\leq t_n=t\}$ of the interval $[s,t]$. For $\lambda \in \N$, we define the dyadic refinement of $P_0$ of order $\lambda$ by $\PP_\lambda := \{t_i + k2^{-\lambda}(t_{i+1}-t_i)\}_{0\leq i\leq n,\ \leq k \leq 2^\lambda}$. We then define the corresponding solution grid $\DD_\lambda := \big(\PP_\lambda\times\PP_\lambda\big) \cap \{s\leq u\leq r\leq t\}$. The normalised quadrature area between two times $(u_i,u_j)\in\DD_\lambda$ is given by
% \[
% (\Delta A)_{i}^j:=\frac{(u_{i+j}-u_i)^2}{(j+1)(j+2)},
% \]
% and we write
% \[
% \langle\Delta_i\gamma,\Delta_j\gamma\rangle
% (\Delta \gamma)_{i}^j:= \frac{\langle \gamma_{u_{i+1}}-\gamma_{u_{i}},\gamma_{u_{j}}-\gamma_{u_{j-1}}\rangle}{(u_{i+1}-u_{i})(u_{j}-u_{j-1})}
% \]
% for the approximation to the inner products of the derivatives of $\gamma$. Note that the derivatives look forward from $u_i$ and backwards from $u_j$. We now define $\hat{K}_\gamma^\lambda:\DD_\lambda\to\R$, to be the solution to the implicit (fully determined) system of equations
% \begin{equation}\label{eq: implicit_system}
% \begin{split}
%      \big(\hat{K}_\gamma^\lambda\big)_{i,{i+j}} =&1 - (\Delta A)_{i}^j\sum_{0\leq k<l\leq j} \hat{K}_\gamma^\lambda(u_i, u_{i+k})\hat{K}_\gamma^\lambda(u_{i+k},u_{i+l})(\Delta \gamma)_{i+k}^{i+l}\\
%      &-(\Delta A)_{i}^j\sum_{0\leq k \leq j}\hat{K}_\gamma^\lambda(u_i,u_{i+k})\hat{K}_\gamma^\lambda(u_{i+k},u_{i+k})(\Delta \gamma)_{i+k-1}^{i+k},
% \end{split},\quad(u_i,u_{i+j})\in\DD_\lambda,
% \end{equation}
% with boundary condition $\hat{K}_\gamma^\lambda(u_i,u_i)=1$ for all $u_i\in \PP_\lambda$. Since $\hat{K}_\gamma^\lambda(u_i,u_{i+j})$ appears only twice on the right-hand side of \cref{eq: implicit_system}, we may use the boundary conditions to rearrange the above to obtain the explicit system of equations
% \small{
% \begin{equation}\label{eq: explicit_system}
%     \hat{K}_\gamma^\lambda(u_i,u_{i+j})=\frac{1 - (\Delta A)_{i}^j\sum\limits_{0\leq k <j}\hat{K}_\gamma^\lambda(u_i,u_{i+k})\left((\Delta \gamma)_{i+k-1}^{i+k} + \sum\limits_{\substack{k<l\leq j\\ (k,j)\neq (0, j)}}\hat{K}_\gamma^\lambda(u_{i+k},u_{i+l})(\Delta \gamma)_{i+k}^{i+l}\right)}{1 - (\Delta A)_{i}^j\left[(\Delta \gamma)_{i}^{i+j}+(\Delta \gamma)_{i+j-1}^{i+j}\right]}.
% \end{equation}
% }
% Since the right-hand side of \cref{eq: explicit_system} only involves certain $\hat{K}_\gamma^\lambda(u_k,u_{l})$ for which $l-k<j$, the system may be solved recursively by first evaluating the solution at $(u_i,u_{i+1})\in\DD_\lambda$ and then at $(u_i,u_{i+2})$ and so on. Solving this system with the most basic implementation would incur a time complexity of $\OO\big(n^4\big)$ in the length of the path. We can reduce this time complexity in two steps. First, we leverage the recursive nature of the equations. For any $s\leq v\leq t$, the system reflects the fact that the integral in the right-hand-side of \cref{eq: func_eq} may be split as
% \begin{align*}
%     K_\gamma(s,t) &= 1-\int_s^v\int_s^r K_\gamma(s, u)K_\gamma(u,r)\langle \dif \gamma_u,\dif \gamma_r\rangle- \int_v^t\int_s^vK_\gamma(s, u)K_\gamma(u,r)\langle \dif \gamma_u,\dif \gamma_r\rangle\\
%     &\quad -\int_v^t\int_v^rK_\gamma(s, u)K_\gamma(u,r)\langle \dif \gamma_u,\dif \gamma_r\rangle\\
%     &=K_\gamma(s, v)- \int_v^t\int_s^vK_\gamma(s, u)K_\gamma(u,r)\langle \dif \gamma_u,\dif \gamma_r\rangle-\int_v^t\int_v^rK_\gamma(s, u)K_\gamma(u,r)\langle \dif \gamma_u,\dif \gamma_r\rangle.
% \end{align*}
% This suggests that the first integral should not need to be approximated, as the integral over this region is already known. Indeed, for $j\geq 2$, it holds that
% \begin{align*}
%     &\sum\limits_{0\leq k <j}\hat{K}_\gamma^\lambda(u_i,u_{i+k})\Bigg((\Delta \gamma)_{i+k-1}^{i+k} + \sum\limits_{\substack{k<l\leq j\\ (k,j)\neq (0, j)}}\hat{K}_\gamma^\lambda(u_{i+k},u_{i+l})(\Delta \gamma)_{i+k}^{i+l}\Bigg)\\
%     =&\frac{1-\hat{K}_\gamma^{\lambda}(u_i,u_{i+j-1})}{(\Delta A)_{i}^{j-1}}+\sum_{0< k < j}\hat{K}_\gamma^\lambda(u_i, u_{i+k})\hat{K}_\gamma^\lambda(u_{i+k},u_{i+j})(\Delta \gamma)_{i+k}^{i+j}.
% \end{align*}
% The resulting sum now involves one free variable and not two; replacing the corresponding sum in \cref{eq: explicit_system}, reduces the time complexity to $\OO\big(n^3\big)$. Just as for the finite difference scheme proposed in \cite{SigPDE} for the ordinary signature kernel, rather than solving the grid in row and column order, we can update a whole anti-diagonal of the solution grid at once since there is no shared dependency between points on the same anti-diagonal. It is possible to exploit this parallelisation using \textrm{GPU} architecture, provided that the length $n$ of $\gamma$ does not exceed the total number of threads on the \textrm{GPU}. The overall time complexity is then $\OO\big(d2^{2\lambda}n^2\big)$ on the grid $\DD_\lambda$.

% For every $N\in\N$ we assume that for $1\leq k\leq 4$
%     \begin{equation}
%         \sup_{N\in\N}\sup_{1\leq m\leq N}\Ex\big[\big\vert{\xi^N(m)\big\vert}^k\big]\leq c_\xi(k)<\infty,
%     \end{equation}
%     and finally that
%     \begin{equation}
%         \Ex\big[\xi_i^N(m)\big] = 0,\quad\text{and}\quad \Ex\big[\xi_i^N(m)^2\big]=1.
%     \end{equation}

% \begin{theorem}\label{thm: L2}
%         Let $(\Omega,\FF,\P)$, $A_i^N$, $\gamma,\sigma$ and $Z_\gamma^N, Z_\sigma^N$ be as in \cref{thm: main_thm}, then
%         \begin{equation}
%             \frac{1}{N}\langle Z_\gamma^N(s),Z_\sigma^N(t)\rangle_\text{HS}\xrightarrow{L_2}\langle \SS_{0,s}(\gamma),\SS_{0,t}(\sigma)\rangle.
%         \end{equation}
% \end{theorem}
% \begin{proof}
%     By expanding
%     \[
%     \Ex\Big[\big(\frac{1}{N}\langle Z_\gamma^N(s),Z_\sigma^N(t)\rangle_{\text{HS}}-\langle \SS_{0,s}(\gamma),\SS_{0,t}(\sigma)\rangle_{\text{HS}}\big)^2\Big]
%     \]
%     in the fashion of \cref{eq: sig_expansion}, we see that the objective is to prove
%     \begin{equation}\label{eq: sig_expansion_quad}
%     \begin{split}
%         \lim_{N\to\infty} \Ex\bigg[&\sum_{|\bm{I}|,|\bm{K}|,|\bm{L}|,|\bm{K}|=0}^\infty \bigg(\frac{1}{N^{\frac{|\bm{I}^\star\bm{J}|}{2}+1}}\tr{A_{\bm{I}\star \bm{J}}^N} -\delta_{\bm{I}\bm{J}}\bigg)\cdot\\
%         &\cdot\bigg(\frac{1}{N^{\frac{|\bm{K}^\star\bm{L}|}{2}+1}}\tr{A_{\bm{K}\star \bm{L}}^N} -\delta_{\bm{K}\bm{L}}\bigg)\hspace{1mm}\SS_{0,s}^{\bm{I}}(\gamma)\SS_{0,t}^{\bm{J}}(\sigma)\SS_{0,s}^{\bm{K}}(\gamma)\SS_{0,t}^{\bm{L}}(\sigma)\bigg]=0.
%     \end{split}
%     \end{equation}
%     As in the proof of \cref{thm: main_thm}, we can show that exchanging the limit and expectation with the quadruple sum is justified. Multiplying out the brackets in \cref{eq: sig_expansion_quad} and taking limits of terms already dealt with in \cref{thm: main_thm} reduces the problem to showing
%     \begin{equation}
%     \begin{split}
%         \sum_{|\bm{I}|,|\bm{K}|,|\bm{L}|,|\bm{K}|=0}^\infty \bigg(\lim_{N\to\infty}&\frac{1}{N^{\frac{|\bm{I}^\star\bm{J}|+|\bm{K}^\star\bm{L}|}{2}+2}}\Ex\Big[ {\xi^N}^\top A_{\bm{I}\star \bm{J}}^N {\xi^N}{\xi^N}^\top A_{\bm{K}\star \bm{L}}^N {\xi^N}\Big]\\
%         &-\delta_{\bm{I}\bm{J}}\delta_{\bm{K}\bm{L}}\bigg)\hspace{1mm}\SS_{0,s}^{\bm{I}}(\gamma)\SS_{0,t}^{\bm{J}}(\sigma)\SS_{0,s}^{\bm{K}}(\gamma)\SS_{0,t}^{\bm{L}}(\sigma)=0.
%     \end{split}
%     \end{equation}
%     By expanding the expectation coordinate-wise, splitting the resulting sum and using the assumptions on $A_i^N$ and $\xi^N$, we can see that the expectation is equal to 
%     \begin{equation}
%     \begin{split}
%          \frac{1}{N^{\frac{|\bm{I}^\star\bm{J}|+|\bm{K}^\star\bm{L}|}{2}+2}}\bigg(&\Ex\Big[\tr{A_{\bm{I}\star \bm{J}}^N}\tr{A_{\bm{K}\star \bm{L}}^N}\Big]+\Ex\Big[\tr{A_{\bm{I}\star \bm{J}}^NA_{\bm{K}\star \bm{L}}^N}+\tr{A_{\bm{I}\star \bm{J}}^N{A_{ \bm{L}\star\bm{K}}^N}}\Big]\\
%          &+\sum_{m=1}^N\Ex\big[A_{\bm{I}\star \bm{J}}^N(m,m)A_{\bm{K}\star \bm{L}}^N(m,m)\big]\Ex\big[(\xi_i^N)^4-3\big]\bigg).
%     \end{split}
%     \end{equation}
%     Noting the scaling factor multiplying all the terms, it is straightforward to apply the techniques of \cref{thm: main_thm} to see that the second and third terms vanish in the limit (the sum of all terms in the expansion of the trace is of order $N^{\frac{n+m}{2}+1}$). Thus it remains to show that
%     \[
%     \lim_{N\to\infty}\frac{1}{N^{\frac{|\bm{I}^\star\bm{J}|+|\bm{K}^\star\bm{L}|}{2}+2}}\Ex\Big[\tr{A_{\bm{I}\star \bm{J}}^N}\tr{A_{\bm{K}\star \bm{L}}^N}\Big]=\delta_{\bm{I}\bm{J}}\delta_{\bm{K}\bm{L}}.
%     \]
%     Given closed words $\bm{w}=w_1\dots w_{n}w_1$ and $\bm{u}=u_1\dots u_m u_{1}$, we define the graphs $G_{\bm{w},\bm{u}}^{u}\coloneqq G_{\bm{w}}^{u}\cup G_{\bm{u}}^{u}$. Now we can write
%     % $\bm{w}\circ\bm{u}\coloneqq w_1\dots w_{n}w_1\circ u_1\dots u_m u_{1}$ to be a closed word of length $k\coloneqq n+m+2$. The use of ``$\circ$'' will reflect the fact that when constructing the graphs $G_{\bm{w}\circ\bm{u}}^{u,d}$, we will not create the edge $\{w_1,u_1\}$, i.e. $G_{\bm{w}\circ\bm{u}}^{u,d}=G_{\bm{w}}^{u,d}\cup G_{\bm{u}}^{u,d}$. Now we can write
%     \begin{equation}
%         \frac{1}{N^{\frac{|\bm{I}^\star\bm{J}|+|\bm{K}^\star\bm{L}|}{2}+2}}\Ex\Big[\tr{A_{\bm{I}\star \bm{J}}^N}\tr{A_{\bm{K}\star \bm{L}}^N}\Big]=\frac{1}{N^{\frac{|\bm{I}^\star\bm{J}|+|\bm{K}^\star\bm{L}|}{2}+2}}\sum_{\bm{w},\bm{u}}\mathscr{C}_{\bm{w},\bm{u}},
%     \end{equation}
%     where $\bm{w}=w_1 w_2\dots w_r w_{r+1} \dots w_n w_{1}$ and $\bm{u}=u_1 u_2\dots u_s u_{s+1} \dots u_m u_{1}$ and
%     \[
%     \begin{split}
%     \mathscr{C}_{\bm{w},\bm{u}}\coloneqq \Ex\bigg[&{A_{i_{|\bm{I}|}}^{N^\top}}(w_1,w_2) \dots {A_{i_1}^{N^\top}}(w_r,w_{r+1}) {A_{j_1}^N}(w_{r+1},w_{r+2})\dots {A_{j_{|\bm{J}|}}^N}(w_{n},w_{1})\\
%         &{A_{k_{|\bm{K}|}}^{N^\top}}(u_1,u_2) \dots {A_{k_1}^{N^\top}}(u_s,u_{s+1}) {A_{l_1}^N}(u_{s+1},u_{s+2})\dots {A_{l_{|\bm{L}|}}^N}(u_{m},u_{1})\bigg].
%     \end{split}
%     \]
%     As in \cref{lem: correct_limit}, $N_{\bm{w},\bm{u}}^e$ must be at least $2$ for every $e\in E_{\bm{w},\bm{u}}^u$ in order for $\mathscr{C}_{\bm{w},\bm{u}}$ to not vanish. This implies that $|E_{\bm{w},\bm{u}}^u|\leq \tfrac{n+m}{2}$, and since $G_{\bm{w},\bm{u}}^{u}$ has at most two connected components, the restriction $\wt{\bm{w}\bm{u}}=|V_{\bm{w},\bm{u}}^u|\leq \tfrac{n+m}{2}+2$ is imposed. Moreover, $\wt{\bm{w}\bm{u}}=\tfrac{n+m}{2}+2$ if and only if $G_{\bm{w},\bm{u}}^{u}$ has two connected components, one with $\frac{n}{2}+1$ vertices and the other with $\frac{m}{2}+1$ vertices; in other words $G_{\bm{w}}^u$ and $G_{\bm{u}}^u$ are disjoint trees. Similar analysis to \cref{lem: correct_limit} shows that only the terms with weight $\tfrac{n+m}{2}+2$ survive in the limit, and in this case
%     \[
% \mathscr{C}_{\bm{w},\bm{u}}=\mathscr{C}_{\bm{w}}\big(A_{\bm{I}\star \bm{J}}^N\big)\mathscr{C}_{\bm{u}}\big(A_{\bm{K}\star \bm{L}}^N\big),
%     \]
%     since the words are disjoint. This reduces the problem to the one handled \cref{lem: correct_limit}. This product will be non-zero if and only if $\bm{I}=\bm{J}$ and $\bm{K}=\bm{L}$. Since there are $N(N-1)\dots \big(N-\tfrac{|\bm{I}^\star\bm{J}|+|\bm{K}^\star\bm{L}|}{2}-1\big)$ members of the equivalence class of $\bm{w}\bm{u}$, it holds that
%     \[
%     \lim_{N\to\infty}\frac{\Ex\Big[\tr{A_{\bm{I}\star \bm{J}}^N}\tr{A_{\bm{K}\star \bm{L}}^N}\Big]}{N^{\frac{|\bm{I}^\star\bm{J}|+|\bm{K}^\star\bm{L}|}{2}+2}}=\lim_{N\to\infty}\frac{N(N-1)\dots \big(N-\tfrac{|\bm{I}^\star\bm{J}|+|\bm{K}^\star\bm{L}|}{2}-1\big)}{N^{\frac{|\bm{I}^\star\bm{J}|+|\bm{K}^\star\bm{L}|}{2}+2}}\delta_{\bm{I}\bm{J}}\delta_{\bm{K}\bm{L}}=\delta_{\bm{I}\bm{J}}\delta_{\bm{K}\bm{L}}.
%     \]
% \end{proof}
% \begin{remark}
%     The assumptions of \cref{thm: main_thm,thm: L2} are satisfied in the case of independent entries of sub-Gaussian random variables under the condition
%     \[
%     \sup_{N\in\N}\sup_{1\leq i \leq d}\sup_{1\leq m,l\leq N} \norm{A_i^N(m,l)}_{\psi}<\infty,
%     \]
%     where $\norm{\cdot}_\psi$ denotes the sub-Gaussian norm. In this case, it is clear that \cref{eq: moment_condition} holds and it can be verified from \cite[Theorem 4.4.5]{Vershynin} that \cref{eq: sub_gaussian_condition} holds.
% \end{remark}
